The Future of Gamma-Ray Experiments in the MeV-EeV Range

Gamma-rays, the most energetic photons, carry information from the far reaches of extragalactic space with minimal interaction or loss of information. They bring messages about particle acceleration in environments so extreme they cannot be reproduced on earth for a closer look. Gamma-ray astrophysics is so complementary with collider work that particle physicists and astroparticle physicists are often one in the same. Gamma-ray instruments, especially the Fermi Gamma-ray Space Telescope, have been pivotal in major multi-messenger discoveries over the past decade. There is presently a great deal of interest and scientific expertise available to push forward new technologies, to plan and build space- and ground-based gamma-ray facilities, and to build multi-messenger networks with gamma rays at their core. It is therefore concerning that before the community comes together for planning exercises again, much of that infrastructure could be lost to a lack of long-term planning for support of gamma-ray astrophysics. Gamma-rays with energies from the MeV to the EeV band are therefore central to multiwavelength and multi-messenger studies to everything from astroparticle physics with compact objects, to dark matter studies with diffuse large scale structure. These goals and new discoveries have generated a wave of new gamma-ray facility proposals and programs. This paper highlights new and proposed gamma-ray technologies and facilities that have each been designed to address specific needs in the measurement of extreme astrophysical sources that probe some of the most pressing questions in fundamental physics for the next decade. The proposed instrumentation would also address the priorities laid out in the recent Astro2020 Decadal Survey, a complementary study by the astrophysics community that provides opportunities also relevant to Snowmass.

==> showerparticledet.tex <==
The extended nature of air showers, where the particle shower front can cover areas of $\mathcal{O}(10^{5} \mathrm{m}^2)$, poses a significant challenge to their detection in a cost-effective manner. Most current and previous instruments that detect air shower particles at ground level use the water Cherenkov technique described in Sec.~\ref{sec:water_cherenkov} but those can be supplemented or completely implemented using other particle-detection techniques such as scintillator arrays (LHAASO, Tibet AS-$\gamma$, ALPACA) or resistive plate chamber (RPC) detectors (e.g. ARGO-YBJ). Scintillator arrays benefit from being light-weight which simplifies their deployment, but given that most detectors are flat and relatively thin their sensitivity drops quickly with the zenith angle $\theta$ of the incoming air shower as their cross-sectional projected onto the shower front drops with $1/\cos{\theta}$.
